A First-Occupancy Representation for Reinforcement Learning

Both animals and artificial agents benefit from state representations that support rapid transfer of learning across tasks and which enable them to efficiently traverse their environments to reach rewarding states. The successor representation (SR), which measures the expected cumulative, discounted state occupancy under a fixed policy, enables efficient transfer to different reward structures in an otherwise constant Markovian environment and has been hypothesized to underlie aspects of biological behavior and neural activity. However, in the real world, rewards may move or only be available for consumption once, may shift location, or agents may simply aim to reach goal states as rapidly as possible without the constraint of artificially imposed task horizons. In such cases, the most behaviorally-relevant representation would carry information about when the agent was likely to first reach states of interest, rather than how often it should expect to visit them over a potentially infinite time span. To reflect such demands, we introduce the first-occupancy representation (FR), which measures the expected temporal discount to the first time a state is accessed. We demonstrate that the FR facilitates exploration, the selection of efficient paths to desired states, allows the agent, under certain conditions, to plan provably optimal trajectories defined by a sequence of subgoals, and induces similar behavior to animals avoiding threatening stimuli.

==> m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecates

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> m.symbols.tex <==
\RequirePackage{ifthen}
\RequirePackage{mathtools}

% use | for math mode
%\catcode`\|=3

% DRL
\newcommand{\Dq}{\stackrel{D}{=}}
\newcommand{\Dqdef}{\stackrel{D}{\coloneqq}}
\newcommand{\bellop}{\mathcal{T}}

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}

% symbols for probability distributions
\newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
\newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
\newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}
% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\lr]{x} -> \mathbb{E}_a \lr[ x \lr]
\makeatletter
\def\expect{\@ifnextchar[{\expect@}{\expect@@[][\lr]}}
\def\expect@[#1]{\@ifnextchar[{\expect@@[#1]}{\expect@@[#1][\lr]}}
\def\expect@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{E}\newlr#2[{#3}#2]}%
             {\mathbb{E}_{#1}\newlr#2[{#3}#2]}}
\def\var{\@ifnextchar[{\var@}{\var@@[][\lr]}}
\def\var@[#1]{\@ifnextchar[{\var@@[#1]}{\var@@[#1][\lr]}}
\def\var@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{V}\newlr#2[{#3}#2]}%
             {\mathbb{V}_{#1}\newlr#2[{#3}#2]}}
\makeatother
\newcommand{\angles}[2][\lr]{{\newlr #1\langle{#2}#1\rangle}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% likelihoods
\newcommand{\like}[2]{\ensuremath{{\cal L}_{#1}\left({#2}\right)}}
\newcommand{\loglike}[2]{\ensuremath{\ell_{#1}\left({#2}\right)}}
\newcommand{\eff}{\mathcal{F}}
% info theoretic
\newcommand{\entropy}[2][\lr]{\ensuremath{\textbf{\textsf{H}}%
                             {\newlr #1[{#2}#1]}}}
\def\mutualinfo[#1;#2]{\ensuremath{\textbf{\textsf{I}}[{#1};{#2}]}}
\newcommand{\KL}[3][\lr]{\ensuremath{\textbf{\textsf{KL}}%
                             {\newlr #1[{#2}\lrmid #1\|{#3}#1]}}}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\newcommand{\normal}[3][\lr]{\ensuremath{\newlr\mathcal{N}#1(#2,#3#1)}}

% fractions
\newcommand{\half}{\ensuremath{{1\over2}}}
\newcommand{\overN}{\ensuremath{{1\over N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}

% whitened quantities
\newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\setV}{\ensuremath{{\cal V}}}
\newcommand{\setX}{\ensuremath{{\cal X}}}
\newcommand{\setY}{\ensuremath{{\cal Y}}}
\newcommand{\setZ}{\ensuremath{{\cal Z}}}
\newcommand{\size}[1]{\ensuremath{\left\vert{#1}\right\vert}}

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\newcommand{\norm}[2][\lr]{\ensuremath{\newlr#1\|#2#1\|}}
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\renewcommand{\det}[2][\lr]{\ensuremath{\newlr#1\vert{#2}#1\vert}}
\newcommand{\trace}[2][\lr]{\ensuremath{\newlr\mathsf{Tr}#1[{#2}#1]}}
\newcommand{\diag}[2][\lr]{\ensuremath{\newlr\mathbox{\textsf{diag}}#1[{#2}#1]}}


% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\newcommand{\intdx}[1][dx]{\int\!\!#1\,}

\newcounter{multintctr}
\newcommand{\mltint}[1][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \int}

\newcommand{\mltintdx}[2][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \intdx[#2]}

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
%\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}


% accents

% adapted from symbols-a4.pdf; optional args permit shortening at left
% and right ends
\makeatletter
\def\widebar{\@ifnextchar[{\widebar@}{\widebar@@[3][0]}}
\def\widebar@[#1]{\@ifnextchar[{\widebar@@[#1]}{\widebar@@[#1][0]}}
\def\widebar@@[#1][#2]#3{{}\mkern#1mu\mkern#2mu\overline{\mkern-#1mu#3\mkern-#2mu}}
\makeatother    
        

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}


\newboolean{inlr}
\newboolean{midlr}
\setboolean{inlr}{false}
\newcommand\newlr{\setboolean{inlr}{false}}

\newcommand\lr[1]{%
  \ifthenelse{\boolean{inlr}}%
    {\ifthenelse{\boolean{midlr}}%
      {\middle#1\setboolean{inlr}{true}}
      {\right#1}}%
    {\left#1\setboolean{inlr}{true}}}%
\newcommand\lrmid{%
  \ifthenelse{\boolean{inlr}}%
    {\setboolean{midlr}{true}}
    {}}%



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

